Exact and Efficient Unlearning for Large Language Model-based Recommendation

The evolving paradigm of Large Language Model-based Recommendation (LLMRec) customizes Large Language Models (LLMs) through parameter-efficient fine-tuning (PEFT) using recommendation data. The inclusion of user data in LLMs raises privacy concerns. To protect users, the unlearning process in LLMRec, specifically removing unusable data (e.g., historical behaviors) from established LLMRec models, becomes crucial. However, existing unlearning methods are insufficient for the unique characteristics of LLM-Rec, mainly due to high computational costs or incomplete data erasure. In this study, we introduce the Adapter Partition and Aggregation (APA) framework for exact and efficient unlearning while maintaining recommendation performance. APA achieves this by establishing distinct adapters for partitioned training data shards and retraining only the adapters impacted by unusable data for unlearning. To preserve recommendation performance and mitigate considerable inference costs, APA employs parameter-level adapter aggregation with sample-adaptive attention for individual testing samples. Extensive experiments substantiate the effectiveness and efficiency of our proposed framework

==> 1_intro_backup_1109.tex <==
\section{introduction}
%Large language models, with their exceptional generative and reasoning abilities, can be fine-tuned to tackle various downstream tasks. However, these models often come with a substantial number of parameters \eg GPT-3, which has 175 billion parameters, and training all of these parameters would involve significant time and resource costs. To address these challenges, recent works have introduced a technique known as "parameter-efficient fine-tuning" (PEFT). This technique entails freezing parts of LLM weights and only updating a subset of model parameters or introducing trainable model components for different downstream tasks. Thanks to PEFT, many individual users and small companies can train their own task-specific language models offline and deploy them online as versatile web application services. Recommendation Systems (RS) represent one such service, empowering language models to generate target items that align with users' preferences or to make inferences regarding user preferences based on the analysis of users' historical interactions with items. Similar to conventional recommendation systems, Language Models for Recommendation (LLM4Rec) often require the ability to forget sensitive information. The process of removing data points from the model is known as "Machine Unlearn," especially within the realm of recommendation systems, where it is referred to as "RecUnlearn." This is of particular significance for large language models employed in recommendation systems and for pretraining-finetuning tasks. These studies have demonstrated that users' sensitive information may potentially be revealed by the trained models.Additionally, LLM4Rec might also need to purge specific problematic data, like out-of-distribution (OOD) data or data compromised by poisoning attacks. Furthermore, evolving user interests or shifting user requirements may require service providers to expunge particular segments of interaction history. To meet these demands, the implementation of "Machine Unlearn" is essential within the framework of LLM4Rec.


%The most straightforward method for unlearning is to retrain from the original data after removing the samples that need to be forgotten. However, even with the employment of the PEFT technique, the cost of retraining can be deemed unacceptable. In the scenario of Machine Unlearn in LLM, current research primarily relies on approximate unlearn methods. These methods often update parameters through gradient-based approaches or directly assess the knowledge gap between the unlearned model and the target model. The issue with these methods is that they cannot guarantee complete unlearning, and it's challenging to completely eliminate the impact of forgotten sample points on the model. Moreover, exact unlearning techniques like data partition cannot be directly applied to LLM4Rec models for the following reasons:(1)During the inference stage, data partition methods aggregate the outputs of sub-models for prediction. For LLM, the time cost of single-model inferencing cannot be overlooked. Simultaneously computing all sub-models is infeasible for LLM web applications. (2)Traditional methods of partitioning datasets cannot be readily adapted to fulfill the partitioning requirements of LLM4Rec.


%To address the issues mentioned earlier and align with the characteristics of using PEFT for LLM4Rec, we introduce a new and efficient erasable framework for PEFT LLM4Rec, which we've named "zyangnb." The fundamental idea behind "zyangnb" is to divide the training dataset into multiple shards and train a submodel for each shard. To mitigate the high computational cost during output aggregation, we draw inspiration from the "mixture of adapters" approach. For each submodel, we train specific PEFT adapters and, during the inference stage, aggregate these PEFT adapters into a personalized adapter. So we only need to use one model to interfere. Previous work on mixtures of adapters has typically followed two main approaches: (1) Assigning the same weights to each adapter, which lacks personalization and can impact the overall model's recommendation effectiveness. (2) Utilizing Mixture of Experts (MoE) techniques to learn dynamic weights for each sample. However, this approach is unpractical in an unlearn scenario, as removing data from a sub-group necessitates retraining a specific submodel, and also requires retraining the relevant MoE parameters, which increases the overall cost.


%In our proposed method, during the inference stage, for each sample point, we construct a neighbor user set by calculating its similarity to the data in the validation set. We then assign weights to the submodels based on their performance within this neighbor user set. During the training phase, we select the model based on its utility on the validation set. Therefore, when an unlearn request is received, we only need to retrain the specific sub-group to assess the utility of the validation set with the new model. This eliminates the need for additional parameters and training costs. Furthermore, regarding data partitioning, we do not rely on collaborative filtering information from the recommendation system. Instead, we use the “language space” information from each instruction for partitioning. We also explore and test two different aggregation methods: 1) "cat" and 2) "soup."To evaluate our method, we apply "zyangnb" to two real-world datasets and conduct extensive experiments. We use "TALLRec" as our base model, which is an LLM4Rec model utilizing the PEFT technique. The experimental results demonstrate that "zyangnb" not only achieves efficient unlearning but also outperforms state-of-the-art unlearning frameworks like SISA, GraphEraser, and RecUnlearn in terms of performance. Further ablation studies confirm the effectiveness of our proposed data partitioning strategies and the "mixture of adapters" method.

%The primary contributions of this work are as follows:
%大型语言模型在多个方面展现出了出色的能力，如通用文本理解和生成，引发了人们对它们在各个领域探索和应用的兴趣。推荐系统，提供了个性化的网络信息过滤，也有望受益于大型语言模型的能力在用户兴趣建模和项目理解等方面获得增强。为了充分解锁这一潜力，研究人员和从业者付出了大量努力使用推荐数据来开发专用于推荐的大型语言模型（称为LLM4Rec），尤其是通过参数高效微调（PEFT）。然而，将推荐特定数据（which通常是用户个人数据如行为数据）的引入可能增加泄露个人数据的风险，考虑到LLM非匿名（文本）化数据记忆及相对开放的prompt记忆激发特点。为了遵守法规保护隐私，及时有效地回应用户要求从微调后大型语言模型中删除他们的个人数据十分重要，激发了一个新的研究问题，即LLM4Rec遗忘。
Large language models (LLMs) have demonstrated exceptional capabilities in various aspects, such as general text comprehension and generation, sparking interest in exploring and applying them in different fields~\cite{llM4med,llM4visual,llM4multimodel}. Recommender systems, one core engine for personalized information filtering, are also expected to benefit from these capabilities in enhancing user modeling, item comprehension~\cite{collm}, etc. To fully unlock this anticipation, researchers and practitioners have dedicated significant effort to develop LLMs specialized for recommendations (referred to as LLM4Rec) with recommendation data, particularly through Parameter-Efficient Fine Tuning (PEFT)~\cite{tallrec,bigrec,collm,yuanfj-adapter}. However, the incorporation of recommendation data (typically user personal data like behavioral data) could increase the risk of personal data leakage, considering the non-anonymous data memory and relatively open memory access characteristics of LLMs~\cite{private1,private2,private3,private4}. To protect privacy, it is crucial to timely and effectively respond to user requests to remove some personal data~\cite{sisa} (termed \textit{unusable data}~\cite{ifru}) from developed LLM4Rec, raising the research question of LLM4Rec unlearning.

% Large language models have showcased remarkable capabilities in various aspects like general text comprehension and generation, kindling excitement for their exploration and application in diverse fields. Recommendation systems, providing personalized information filtering on the web, are also anticipated to harness the capabilities of LLMs in enhancing user interest modeling and item understanding. To fully unlock the anticipation, researchers and practitioners have dedicated significant effort to developing LLMs for recommendation (LLM4Rec) using recommendation data, particularly through a Parameter-Efficient Fine Tuning (PEFT) manner. However, the involvement of recommendation-specific data (e.g., user behavior data) in LLMs would increase the potential of leaking personal data, given the LLMs' strong ability of non-anonymity style (i.e., text style) data memory and open access. To preserve privacy as regulations require, it is critical to effectively and timely respond to user requests to erase their personal data from the tuned LLM, raising a new question of LLM4Rec unlearning. 

% Large language models(LLMs), known for their impressive capabilities in generating content and reasoning, have sparked enthusiasm for exploration in various domains. To effectively tune these models to tasks in diverse fields, domain-specific Parameter-Efficient Fine-Tuning (PEFT) has become the dominant paradigm in the industry. Recommendation systems (RS), a fundamental component of today's internet infrastructure, have also joined this trend. There is a growing exploration of using LLMs in recommendation systems, often referred to as LLM4Rec. In this process, LLMs not only acquire recommendation capabilities but also accumulate a wealth of domain knowledge related to user-item interactions. When the training dataset contains sensitive information, attackers can easily exploit the characteristics of this data to launch attacks. Previous research has shown that recommendation systems and language models with pretraining-finetuning structures are often more vulnerable to attacks involving sensitive data. Therefore, both users and model owners of LLM4Rec are more urgently in need of data "forget" services.

% 虽然传统unlearning 获得了充分发展，开发了基于梯度的近似unlearning以及基于retraining 的exact unlearning方法。然而，由于LLM 的large size 等特性，LLM realted unlearning unlearning面临着新的挑战，特别是在efficiency方面，还亟待发展。据我们所知目前没有专门研究LLM4Rec unlearning的工作，只是一些关于LLM遗忘pretaining知识的同期研究~cite{InContextUnlearn}。受限于retraining的成本，这些方法基于上下文学习或扩展传统的基于梯度的方法来实现近似遗忘。然而，与LLM遗忘中清除开放世界知识不同，LLM4Rec遗忘中要删除的是个人数据，对于这类数据来说，近似遗忘是不太可接受的。因此，本研究追求对LLM4Rec的精确遗忘。



Research on unlearning has made significant strides with traditional models, establishing mature technical approaches categorized into approximate unlearning and retraining-based exact unlearning~\cite{unlearninSurvey}. However, the large-scale nature of LLMs presents fresh challenges in the field of LLM-related unlearning, particularly concerning efficiency, necessitating further investigation. To our knowledge, there is currently no dedicated research on LLM4Rec unlearning, with only some concurrent work focusing on unlearning LLMs themselves~\cite{InContextUnlearn,HarryUnlearning,yao2023large}. Given the substantial cost associated with LLM retraining, these methods primarily follow the technical path of approximate unlearning to ensure unlearning efficiency, utilizing in-context learning or the extension of traditional techniques.
In contrast, unlike the data typically related to open-world knowledge when unlearning LLMs themselves, LLM4Rec unlearning is concerned with the removal of personal data. In this context, incomplete removal of personal data poses significant risks, including potential regulatory violations, emphasizing the necessity for efficient and exact unlearning.




   

% This article addresses the issue of unlearning in the scenario of LLM4Rec under the PEFT framework. Previous research efforts aimed at exploring LLMs unlearning can be categorized as approximate unlearning and do not provide a guarantee of achieving complete unlearning. Consequently, eliminating the entire influence of sensitive data becomes a challenging task. Our primary objective in unlearning is to ensure comprehensive privacy protection for users. To achieve this goal, we employ data partition techniques as a means to achieve full unlearning. Data partition is a partial retraining-based method. It first divides the training set into several shards. Then, it trains submodels for different shards, and aggregates all submodel outputs as the final prediction.

With the extensive adoption of PEFT in LLM4Rec~\cite{tallrec,bigrec,collm,yuanfj-adapter}, this study is dedicated to achieving exact and efficient unlearning for PEFT-based LLM4Rec with maintaining high recommendation performance. Drawing on insights from traditional unlearning models, retraining has emerged as a reliable method to ensure exact unlearning. Moreover, by implementing a partitioning strategy---dividing the training data into disjoint shards and training distinct sub-models for each shard---efficiency can be maintained by retraining only a small portion of the sub-models affected by unusable data. In the context of PEFT-based LLM4Rec, personal data would be only memorized by the PEFT adapter, enabling us to execute partitioning and retraining exclusively for the adapter. The retraining cost for the adapter is considerably lower than that of the entire model. Furthermore, the adapter's ability to learn rapidly with a minimal number of examples~\cite{tallrec} allows us to further reduce the shard size, ultimately diminishing the retraining cost. These considerations drive us to leverage this partition-empowered retraining approach for LLM4Rec unlearning. 

% When applying the partition strategy, at inference, we usually need to aggregate the prediction of sub-models, to maintain high recommendation performance. For traditional models, the process can be easily executed. However, it is non-trivial for LLMs. The inference of LLMs is computationally expensive, which is much higher than traditional models; and the prediction of the $K$ sub-models would lead to $K$ times inference costs, which would not only significantly intensify energy consumption but also lead to serious latency issues, injuring user experiences. We argue that aggregation is not necessary to perform aggregation after getting a prediction. 
% Instead, we could directly aggregate the weights of sub-models (adapters) to form a single model, making only one-pass inference needed. Once the adapters' weights are not in conflict but Complementary~\cite{modelsoup} and the weights aggregation is suitable, it could also effectively fusion the knowledge of different adapters, boosting the recommendation performance. 

When implementing the partition strategy in LLM4Rec, a distinct inference latency challenge emerges. Typically, during inference, aggregating prediction results from sub-models is necessary to integrate knowledge for maintaining high recommendation performance~\cite{sisa,receraser,graphunlearn}.  However, for LLM4Rec, this aggregation is infeasible, primarily due to the computationally expensive nature of LLM inference~\cite{costhigh}. Generating predictions from $K$ sub-models (adapters) would result in a $K$ times increase in the inference cost of LLMs, which would lead to a substantial rise in energy consumption and cause severe latency issues that can negatively impact the user experience. For this challenge, we contend that aggregation at the prediction result level is unnecessary. If the weights of sub-models (adapters) are not homogenous, directly performing suitable weight aggregation can effectively integrate knowledge from different adapters~\cite{modelsoup}. Therefore, we can aggregate the weights of adapters (termed \textit{soup}~\cite{modelsoup}) to fuse knowledge and create a single model, enabling a single-pass inference with keeping performances.

% To this end, we propose a novel and efficient erasable LLM4Rec framework --- \textit{\textbf{Adapter} \textbf{P}artition and \textbf{S}oup} (AdapterPS), which trains different adapters for divided training data shards and inferences with the adapter weight aggregation. To ensure the aggregateability of the adapters, we divide the training data into balanced shards with different semantics, obtaining heterogeneous data and further making adapters trained on them heterogeneous. Regarding aggregation, we take a sample-specific method --- for each testing sample, we merge the adapter weights based on its most semantically similar validation samples, using the validation performances on different adapters to assign aggregation weights for different adapters. By assigning higher weights to adapters with higher performance, we could pay more attention to adapters suitable for dealing with the sample, ensuring better performance. Moreover, our aggregation is training-free for achieving adaptive aggregation, which would not increase further unlearning costs unlike the prediction aggregation in traditional unlearning. 

To this end, we introduce a novel and efficient erasable LLM4Rec framework, named \textit{\textbf{Adapter} \textbf{P}artition\&\textbf{S}oup} (AdapterPS). This framework trains individual adapters for each partitioned training data shard and leverages adapter weight aggregation during inference, ensuring both unlearning and inference efficiency. To ensure the aggregateability of the adapters, we divide the training data into balanced shards with text semantic characteristics~\cite{bigrec}, making them heterogeneous. This heterogeneity makes the adapters trained on them suitable for aggregation. When performing aggregation, we employ a sample-adaptive approach. For each testing sample, we combine adapter weights based on its most semantically similar validation samples, using the validation performance of different adapters to assign aggregation attention. This allocation prioritizes higher-performing adapters to enhance overall performance. Notably, our aggregation method achieves adaptive aggregation without the need for additional training, unlike prediction aggregation in traditional unlearning~\cite{receraser}, avoiding introducing additional unlearning costs.

The main contributions can be summarized as follows:
\begin{itemize}[leftmargin=*]
    \item New problem:  To our knowledge, this is the first study to formulate and explore exact unlearning within the realm of LLM4Rec.
    \item New technique: We introduce the AdapterPS method, an extension of partition-based unlearning, tailored to scenarios where inference involves high computational costs.
    \item Experiments: We conduct extensive experiments on two real-worlds, verifying the effectiveness of the proposal.
\end{itemize}

% Besides the need to finish unlearning efficiently and exactly, the unlearning process also needs to maintain high recommendation performance. This raises the need to
% \%\%\%\%\%\%\%\%\%\%\%\%\%\%
% \%\%\%\%\%\%\%\%\%\%\%\%\%\%
% \%\%\%\%\%\%\%\%\%\%\%\%\%\%
% \%\%\%\%\%\%\%\%\%\%\%\%\%\%
% \\




% However, when compared to traditional recommendation systems, the implementation of data patition in LLM4Rec encounters notable challenges. The process of retraining each submodel and running multiple submodels for aggregation leads to significant overhead, which is not in line with the principle of "environmental sustainability." While the few-shot capability of LLMs can help reduce the retraining cost for submodels by decreasing the size of subgroups, the aggregation process is still hindered by the significant computational cost associated with large model inference. Each inference operation takes approximately 40 seconds, requiring model loading and content generation, leading to latency issues that can negatively impact the user experience. Thus, practical applications face considerable challenges.

% In line with previous research, we propose an alternative approach: rather than aggregating the output of models, we aggregate the parameters of the PEFT models. This way, during the inference phase, we only need to execute model loading and generation once. However, the process of aggregating models is non-trivial. We cannot afford a significant drop in recommendation performance due to aggregation. This challenge can be addressed through: 1) Proper data partitioning: Ensuring that each submodel learns relevant knowledge, which allows the ability of small-data models to aggregate with large-data models. 2)Reasonable weight Assignment: Many approaches employ methods similar to the Mixture of Experts (MoE) to learn weights, but this can add extra training and retraining costs.

% To tackle the challenges outlined earlier, we introduce a novel and efficient erasable framework for PEFT-based LLM4Rec, which we've named "zyangnb." Our approach combines two key strategies. Firstly, we make use of "language space" information within the instructions for data partitioning. Secondly, we aggregate submodels based on the most similar samples from the validation set and their performance on submodels. Models with better performance receive higher weights. Data partitioning ensures the consistency of different sub-groups, establishing a solid foundation for weighted steps. During model training, we select models based on their performance on the validation set, ensuring effective aggregation without incurring additional costs. Additionally, we explore and test two different aggregation methods: 1) "cat" and 2) "soup."To assess the effectiveness of our method, we conduct extensive experiments by applying "zyangnb" to two real-world datasets. Our base model is "TALLRec," an LLM4Rec model that utilizes PEFT technology. The experimental results clearly demonstrate that "zyangnb" not only achieves efficient unlearning but also outperforms state-of-the-art unlearning frameworks such as SISA, GraphEraser, and RecUnlearn in terms of performance. Further studies that analyze the impact of our data partition strategies and the "mixture of adapters" method provide additional confirmation of their effectiveness. 

% The primary contributions of this work can be summarized as follows:







==> backup/1_intro.tex <==
\section{introduction}
%Large language models, with their exceptional generative and reasoning abilities, can be fine-tuned to tackle various downstream tasks. However, these models often come with a substantial number of parameters \eg GPT-3, which has 175 billion parameters, and training all of these parameters would involve significant time and resource costs. To address these challenges, recent works have introduced a technique known as "parameter-efficient fine-tuning" (PEFT). This technique entails freezing parts of LLM weights and only updating a subset of model parameters or introducing trainable model components for different downstream tasks. Thanks to PEFT, many individual users and small companies can train their own task-specific language models offline and deploy them online as versatile web application services. Recommendation Systems (RS) represent one such service, empowering language models to generate target items that align with users' preferences or to make inferences regarding user preferences based on the analysis of users' historical interactions with items. Similar to conventional recommendation systems, Language Models for Recommendation (LLM4Rec) often require the ability to forget sensitive information. The process of removing data points from the model is known as "Machine Unlearn," especially within the realm of recommendation systems, where it is referred to as "RecUnlearn." This is of particular significance for large language models employed in recommendation systems and for pretraining-finetuning tasks. These studies have demonstrated that users' sensitive information may potentially be revealed by the trained models.Additionally, LLM4Rec might also need to purge specific problematic data, like out-of-distribution (OOD) data or data compromised by poisoning attacks. Furthermore, evolving user interests or shifting user requirements may require service providers to expunge particular segments of interaction history. To meet these demands, the implementation of "Machine Unlearn" is essential within the framework of LLM4Rec.


%The most straightforward method for unlearning is to retrain from the original data after removing the samples that need to be forgotten. However, even with the employment of the PEFT technique, the cost of retraining can be deemed unacceptable. In the scenario of Machine Unlearn in LLM, current research primarily relies on approximate unlearn methods. These methods often update parameters through gradient-based approaches or directly assess the knowledge gap between the unlearned model and the target model. The issue with these methods is that they cannot guarantee complete unlearning, and it's challenging to completely eliminate the impact of forgotten sample points on the model. Moreover, exact unlearning techniques like data partition cannot be directly applied to LLM4Rec models for the following reasons:(1)During the inference stage, data partition methods aggregate the outputs of sub-models for prediction. For LLM, the time cost of single-model inferencing cannot be overlooked. Simultaneously computing all sub-models is infeasible for LLM web applications. (2)Traditional methods of partitioning datasets cannot be readily adapted to fulfill the partitioning requirements of LLM4Rec.


%To address the issues mentioned earlier and align with the characteristics of using PEFT for LLM4Rec, we introduce a new and efficient erasable framework for PEFT LLM4Rec, which we've named "zyangnb." The fundamental idea behind "zyangnb" is to divide the training dataset into multiple shards and train a submodel for each shard. To mitigate the high computational cost during output aggregation, we draw inspiration from the "mixture of adapters" approach. For each submodel, we train specific PEFT adapters and, during the inference stage, aggregate these PEFT adapters into a personalized adapter. So we only need to use one model to interfere. Previous work on mixtures of adapters has typically followed two main approaches: (1) Assigning the same weights to each adapter, which lacks personalization and can impact the overall model's recommendation effectiveness. (2) Utilizing Mixture of Experts (MoE) techniques to learn dynamic weights for each sample. However, this approach is unpractical in an unlearn scenario, as removing data from a sub-group necessitates retraining a specific submodel, and also requires retraining the relevant MoE parameters, which increases the overall cost.


%In our proposed method, during the inference stage, for each sample point, we construct a neighbor user set by calculating its similarity to the data in the validation set. We then assign weights to the submodels based on their performance within this neighbor user set. During the training phase, we select the model based on its utility on the validation set. Therefore, when an unlearn request is received, we only need to retrain the specific sub-group to assess the utility of the validation set with the new model. This eliminates the need for additional parameters and training costs. Furthermore, regarding data partitioning, we do not rely on collaborative filtering information from the recommendation system. Instead, we use the “language space” information from each instruction for partitioning. We also explore and test two different aggregation methods: 1) "cat" and 2) "soup."To evaluate our method, we apply "zyangnb" to two real-world datasets and conduct extensive experiments. We use "TALLRec" as our base model, which is an LLM4Rec model utilizing the PEFT technique. The experimental results demonstrate that "zyangnb" not only achieves efficient unlearning but also outperforms state-of-the-art unlearning frameworks like SISA, GraphEraser, and RecUnlearn in terms of performance. Further ablation studies confirm the effectiveness of our proposed data partitioning strategies and the "mixture of adapters" method.

%The primary contributions of this work are as follows:
Large language models(LLMs), known for their impressive capabilities in generating content and reasoning, have sparked enthusiasm for exploration in various domains.To effectively tune these models to tasks in diverse fields, domain-specific Parameter-Efficient Fine-Tuning (PEFT) has become the dominant paradigm in the industry. Recommendation systems (RS), a fundamental component of today's internet infrastructure, have also joined this trend. There is a growing exploration of using LLMs in recommendation systems, often referred to as LLM4Rec. In this process, LLMs not only acquire recommendation capabilities but also accumulate a wealth of domain knowledge related to user-item interactions. When the training dataset contains sensitive information, attackers can easily exploit the characteristics of this data to launch attacks. Previous research has shown that recommendation systems and language models with pretraining-finetuning structures are often more vulnerable to attacks involving sensitive data. Therefore, both users and model owners of LLM4Rec are more urgently in need of data "forget" services.


This article addresses the issue of unlearning in the scenario of LLM4Rec under the PEFT framework. Previous research efforts aimed at exploring LLMs unlearning can be categorized as approximate unlearning and do not provide a guarantee of achieving complete unlearning. Consequently, eliminating the entire influence of sensitive data becomes a challenging task. Our primary objective in unlearning is to ensure comprehensive privacy protection for users. To achieve this goal, we employ data partition techniques as a means to achieve full unlearning.Data partition is a partial retraining-based method. It first divides the training set into several shards. Then, it trains submodels for different shards, and aggregate all submodel outputs as final prediction.

However, when compared to traditional recommendation systems, the implementation of data patition in LLM4Rec encounters notable challenges. The process of retraining each submodel and running multiple submodels for aggregation leads to significant overhead, which is not in line with the principle of "environmental sustainability." While the few-shot capability of LLMs can help reduce the retraining cost for submodels by decreasing the size of subgroups, the aggregation process is still hindered by the significant computational cost associated with large model inference. Each inference operation takes approximately 40 seconds, requiring model loading and content generation, leading to latency issues that can negatively impact the user experience. Thus, practical applications face considerable challenges.

In line with previous research, we propose an alternative approach: rather than aggregating the output of models, we aggregate the parameters of the PEFT models. This way, during the inference phase, we only need to execute model loading and generation once. However, the process of aggregating models is non-trivial. We cannot afford a significant drop in recommendation performance due to aggregation. This challenge can be addressed through: 1)Proper data partitioning: Ensuring that each submodel learns relevant knowledge, which allows the ability of small-data models to aggregate with large-data models. 2)Reasonable weight Assignment: Many approaches employ methods similar to the Mixture of Experts (MoE) to learn weights, but this can add extra training and retraining costs.

To tackle the challenges outlined earlier, we introduce a novel and efficient erasable framework for PEFT-based LLM4Rec, which we've named "zyangnb." Our approach combines two key strategies. Firstly, we make use of "language space" information within the instructions for data partitioning. Secondly, we aggregate submodels based on the most similar samples from the validation set and their performance on submodels. Models with better performance receive higher weights. Data partitioning ensures the consistency of different sub-groups, establishing a solid foundation for weighted steps. During model training, we select models based on their performance on the validation set, ensuring effective aggregation without incurring additional costs. Additionally, we explore and test two different aggregation methods: 1) "cat" and 2) "soup."To assess the effectiveness of our method, we conduct extensive experiments by applying "zyangnb" to two real-world datasets. Our base model is "TALLRec," an LLM4Rec model that utilizes PEFT technology. The experimental results clearly demonstrate that "zyangnb" not only achieves efficient unlearning but also outperforms state-of-the-art unlearning frameworks such as SISA, GraphEraser, and RecUnlearn in terms of performance. Further studies that analyze the impact of our data partition strategies and the "mixture of adapters" method provide additional confirmation of their effectiveness. 

The primary contributions of this work can be summarized as follows:







==> backup/2_pre.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\label{rec-tuning}
\begin{table}[]
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Instruction Input}}                                                                                                                                              \\ \midrule
Instruction: & \begin{tabular}[c]{@{}l@{}}Given the user's preference and unpreference, indentify\\ whether the user will like the target moive by answering\\ "Yes." or "No."\end{tabular} \\ \midrule
Input:       & \begin{tabular}[c]{@{}l@{}}User preference: Inception  \\ User unpreference: No Country for Old Men\\ Target new movie: Interstellar\end{tabular}                            \\ \midrule
\multicolumn{2}{c}{\textbf{Instruction Output}}                                                                                                                                             \\ \midrule
Output:      & Yes.                                                                                                                                                                         \\ \bottomrule
\end{tabular}

\caption{todo}
\end{table}
\section{Preliminaries}


In this section, we will begin by introducing LoRA, an alternative approach to PEFT. Following that, we will provide a brief overview of our foundational LLM4Rec model, TALLRec. Finally, we will give the formulation of our LLM4Rec unlearning task.


\subsection{LoRA}
Fine-tuning a Large Language Model (LLM) with all parameters can be a resource-intensive and time-consuming process. Parameter-Efficient Fine-Tuning (PEFT) offers a solution to this challenge by adapting only specific parameters or introducing external modules for new tasks. One approach within the PEFT framework is Low-Rank Adaptation (LoRA).

The core idea behind LoRA is to update only the LoRA-specific parameters during the fine-tuning process while keeping all other parameters of the LLM frozen. LoRA comprises two smaller matrices, referred to as update matrices, as illustrated in Figure~\ref{fig:LoRA}. For a weight matrix of an LLM layer, denoted as $\mathcal{W}_0 \in\mathbb{R}^{d\times k}$, we achieve an update through a low-rank decomposition,$\mathcal{W}_0 + \triangle\mathcal{ W} = \mathcal{W}_0 + BA$. Here, $B \in\mathbb{R}^{d\times r}$, $A \in\mathbb{R}^{r\times d}$, and the rank $r \ll min(d,k)$. For a given input $x$, we use both $\mathcal{W}_0$ and $\triangle\mathcal{W}$ to multiply $x$ and then sum the resulting output vectors coordinate-wise. For a layer in the network that incorporates LoRA, its output $h$ is defined as follows:
\begin{equation}\small\label{eq:retraining-loss} 
 h = \mathcal{W}_{0}x + \triangle\mathcal{W}x = \mathcal{W}_{0}x + BAx
\end{equation}
Additionally, LoRA utilizes random Gaussian initialization for $A$ and sets $B$ to zero, which results in an initial value of $\triangle\mathcal{W}=BA$ being zero at the start of training.



\begin{figure}[h]
  \includegraphics[width=1.2\linewidth]{LoRA.pdf}
   \vspace{-10pt}
  \caption{todo}
  \label{fig:LoRA}\vspace{-15pt}
\end{figure}

\subsection{TALLRec}
TALLRec leverages Instruction Tuning and the LoRA structure to empower LLMs with recommendation capabilities. Instruction Tuning is a pivotal technique involving the training of LLMs using human-annotated instructions and responses. TALLRec is built upon the LLaMA-7B model and comprises two distinct tuning stages: alpaca tuning and rec-tuning.

First, let's explore alpaca tuning. During this stage, LLMs are trained using self-instruct data provided by Alpaca, which serves to enhance their generalization ability.

To understand how recommendation data is structured for instruction tuning, it's essential to examine the format. As depicted in Table~\ref{rec-tuning}, TALLRec initiates the process by constructing an "Instruction" that instructs the model to analyze a user's historical interactions, determining whether the user likes a particular target item and responding with either "yes" or "no." The "Input" specifies two categories of historical interactions: those that the user likes and those that the user does not like. Besides, “Input” also includes a target new item that the user has never seen. Finally, the "Output" contains the actual information indicating whether the user likes the target item. In preparation for rec-tuning, TALLRec combines the "Instruction" and "Input" to create "Instruction Input" and sets the expected "Output" as either 'Yes" or "No."

Similar to the approach used in alpaca tuning, TALLRec employs the conditional language modeling objective during the rec-tuning stage.
\begin{equation}\small
\mathop{\max}\limits_{\Theta} \sum_{(x,y)\in\mathcal{Z}}\sum_{t=1}^{|y|}log(P_{\Theta+\Phi}(y_{t}|x,y_{<t}))
\end{equation}
where $x$ and $y$ represent "Instruction Input" and "Output" in rec-tuning Instruction data. Here, $y_{t}$ corresponds to the $t$-th token of the $y$, $y_{<t}$ represents the tokens that precede $y_{t}$, $\Phi$ stands for the parameters of LLMs, and $\mathcal{Z}$ denotes the training set. $\Theta$ is the parameters of LoRA, TALLRec only update the LoRA parameters during the rec-tuning process. 

As the alpaca tuning process doesn't incorporate recommendation information, in the subsequent discussion, all submodels are individually subjected to different rec-tuning processes on the same model that has previously undergone alpaca tuning.

\subsection{Problem Formulation}
When a user $u$ want to forget a interaction record with item $i$,
a LLM4Rec system needs to modify the "Instruction Input" $x_u$ of $u$, and genrate new "Instruction Input" $x_u^{'}$. Making the training set $\mathcal{Z}$ to $\mathcal{Z}^{'}$, and obtain an unlearned model train on $\mathcal{Z}^{'}$.


==> backup/3_method.tex <==
\section{Methodology}

In this section, we will start with an overview of our method. Subsequently, we will introduce a data partition approach based on semantic embedding similarity. Then, we will explain the model aggregation method based on model soup, and provide definitions for two different levels: 1) Lora parameters level and 2) Lora layers level. Finally, we will offer detailed explanations of the sample-adaptive approach.
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{framework.pdf}
   \vspace{-10pt}
  \caption{todo}
  \label{fig:framework}\vspace{-15pt}
\end{figure*}
\subsection{Overview}
The overall workflow of AdapterPS is depicted in Figure~\ref{fig:framework}, which can be divided into three main phases: semantic data partition, submodel training, and weighted PEFT model soups. The semantic data partition part is designed to split the training data into $k$ shards, where the data in the $i$-th shard constitutes the dataset $D_{i}$. After data partitioning, each shard ($D_{i}$) trains a model ($M_{i}$). These models share the same LLMs part, with the sole distinction lying in their PEFT model components. Furthermore, these models can be trained in parallel, which accelerates the training process. During the inference stage, we aggregate the PEFT models of all submodels into model soups using a testing sample-adaptive approach which weighted different adapters based on similar validation performance.

When a forget request is needed, only one of the submodels, whose shard contains the point to be unlearned, needs to be retrained. During retraining, the performance of the new submodel on the validation set is updated, without incurring any extra overhead.
\begin{algorithm}[t]
	\caption{semantic partition algorithm}
	\LinesNumbered
	\label{alg:partiton}
	\KwIn{ Instruction Input $\{x_0,...,x_M\}$ , Instruction Input ’ semantic embeddings $\{e_0,...,e_M\}$, number shards $K$, maximum number of each shard $t$}
 	\KwOut{The Shards $D=\{D_{0},D_{1},...,D_{k}\}$}
   Using kmeans algorithm to generate $K$ anchors $A=\{a_{0},a_{1},...,a_{K}\}$\;
    
    \For{ each $a_{i} \in A $}{
    \For{ each $e_{j} \in E$}{
        calculate $dist(e_{j}-a_{i})$ by eq(4) or eq(5) and store in $F$
    }
    }
    Sort $F$ in ascending order to get $F_{s}$,
   
    Empty $D$

    \For{each $(e_{i},a_{j})$ in $F_{s}$}{
    \If{$|D_{j}|<t$}{
    $S_{j} \leftarrow D_{j} \cup x_{i}$
    }
    }
    return $D$;
\end{algorithm}
\subsection{semantic data partition}
The previous data partition methods relied on dividing data through k-means of node embeddings, user embeddings, item embeddings, or user-item interactions to ensure the effectiveness of grouping. However, language models may be confused in understanding the information applied to grouping. Therefore, inspired by previous work~\cite{bigrec}, our data partition method is based on semantic information similarity, which is more flexible for LLM4Rec tasks.

%The term "language space" refers to a conceptual space that encompasses all possible language sequences that a Large Language Model (LLM) could generate. It represents the vast range of textual outputs or language expressions that the LLM is capable of producing.
When given an input, an LLM generates a corresponding output, and we use the hidden states of the LLM's last layer at the last time step to represent the semantic information of this input. In the context of recommendation tasks, for a model that hasn't undergone rec-tuning, an Instruction Input $x_i$' semantic embedding is defined as follows:
\begin{equation}\small
 e_{i} = hidden_{\Theta}(x_{i})
\end{equation}
Where $\Theta$ represents the model after alpaca tuning and $e_i$ is the initial understanding of the various Instruction Input samples by the initial LLMs. Therefore, the datasets are divided based on the similarity of semantic embeddings to let different models with different semantic characteristics, making them heterogeneous. This will be helpful for the subsequent weighted model soup aggregation process. The specific partitioning algorithm is shown in Algorithm~\ref{alg:partiton}. Given an entire Instruction Input set $\{x_{0},x_{1},...,x_{M}\}$ and their corresponding semantic embeddings $\{e_{0},e_{1},...,e_{M}\}$, K shards are first generated by the k-means algorithm. However, since k-means cannot guarantee balanced grouping, using this grouping directly would result in variations in the effectiveness of each submodel due to differences in data volume. To achieve balanced grouping, we retained the center point $A=\{a_0,...,a_K\}$ of each cluster, and following the setting of k-means, the Euclidean distance is used to calculate the distance between $x_j$ and a particular center point $a_i$:
\begin{equation}\small
    dist(e_{j},a_i) = ||e_{j}-a_{i}||_{2} = \sqrt{\sum_{l=0}^{n}(e_{j,l}-a_{i,l})^2 } 
\end{equation}
Also, we use function $cos(\cdot,\cdot)$ represents the cosine similarity to define the distance between $x_j$ and $a_i$:
\begin{equation}\small
    dist(e_{j},a_i) = -cos(e_{j},a_{i})
\end{equation}
By calculating the distance between each Input Instruction and each center point, we generate an $M\times K$ matrix of distances, which we denote as set F, where $M$ represents the number of Instruction I. Subsequently, we arrange F in ascending order to obtain Fs. For each user-anchor pair in $F_s$, if the size of $D_i$ is smaller than the maximum number of shards $t$, then the Instruction Inputs $x_j$ are allocated to shard $D_i$.

\subsection{model soup}
Model soups is a method for averaging the weights of different models. In our scenario, We don't need to make a soup for the entire model, we only need to make a soup for each model's LoRA, for all submodels sharing the same LLMs parameters. Consider a set of $K$ LoRA trained on different shards, where $B_{ij} \in\mathbb{R}^{d\times r}$, $A_{ij} \in\mathbb{R}^{r\times d}$ represent the update matrix of the $j$th layer of LoRA for the $i$th submodel. So, according to the original model soup method, we have:
\begin{equation}\small
\begin{split}
& h_{j} = \mathcal{W}_{j}x + B_{j}^{'}A_{j}^{'}x \\
& B_{j}^{'} = \frac{1}{K}\ \sum_{i=0}^K\of B_{ij},A_{j}^{'} = \frac{1}{K}\ \sum_{i=0}^K\of A_{ij} \\
\end{split}
\end{equation}
Here $B_{j}^{'}$ and $A_{j}^{'}$ represent the model soups for $j$th Layer's LoRA. And $h_{j}$ denotes as $j$th layer output which uses the new LoRA model soups. However, directly applying an average-weighted model soup may result in a reduction in recommendation performance. To make full use of the unique characteristics of each LoRA model, the Lora parameters level model soup is modified to:
\begin{equation}\small \label{soup}
\begin{split}
& B_{j}^{'} =  \sum_{i=0}^K\of w_{i}B_{ij},A_{j}^{'} =  \sum_{i=0}^K\of w_{i}A_{ij} \\
\end{split}
\end{equation}
Where $w_{i}$ is the weight of $i$th LoRA, and we will provide a detailed explanation in Section 3.4. To understand model soup from another perspective of model aggregation, we introduce a matrix concatenation method:
\begin{equation}\small \label{cat}
\begin{split}
& h_{j} = \mathcal{W}_{j}x + B_{j}^{'}A_{j}^{'}x \\
& B_{j}^{'} =  \begin{bmatrix}
    w_{0}B_{0j} & w_{1}B_{1j} & ... & w_{K}B_{Kj}
\end{bmatrix} \\
& A_{j}^{'} =  \begin{bmatrix}
    A_{0j} & A_{1j}  & ... & A_{Kj}
\end{bmatrix}^{T} \\
\end{split}
\end{equation}
Where $B_{j}^{'}\in\mathbb{R}^{d\times Kr}$ and $A_{j}^{'}\in\mathbb{R}^{Kr\times d}$ represent the new matrix from matrix concatenation, effectively transforming the original rank $r$ of LoRA update matrix into $rK$. It can be mathematically proven that:
\begin{equation}\small
\begin{split}
 h_{j} &= \mathcal{W}_{j}x + B_{j}^{'}A_{j}^{'}x \\
       &= \mathcal{W}_{j}x + \sum_{i=0}^K\of  w_{ij}B_{ij}^{'}A_{ij}^{'}x
\end{split}
\end{equation}
This indicates that the model soup using matrix concatenation is, in fact, aggregating the outputs of different submodels for each layer separately, so, we refer to this form of model soup as the Lora layers level model soup. However, the matrix concatenation approach avoids the additional overhead brought about by loading the LLMs multiple times.
\subsection{testing sample-adaptive approach}
Once the training data is partitioned, a submodel $M_i$ is trained on each shard data $S_i$. To leverage the heterogeneity of the groups effectively, when dealing with a new test Instruction Input $x_i$, it becomes essential to allocate appropriate weights to the adapters based on the characteristics of $x_i$ to achieve a highly effective recommendation. The most straightforward approach is to assign higher weights to adapters that perform well on Instruction Input samples similar to $x_i$. In our framework, for each test instruction input, we select a set of similar samples from the validation set based on the instruction input's similarity:
\begin{equation}\small
\begin{split}
    & \mathcal{N}_{x_i} = \{x_j|x_j \in topk(sim(e_i,e_j) , x_j \in valid\}\\
    & sim(x_i,x_j) = cos(x_i,x_j) or sim(x_i,x_j) = ||x_i,x_j||_{2}
\end{split}
\end{equation}
where $\mathcal{N}_{x_i}$ is the set of Topk similar Instruction Inputs samples in the validation set. We use cosine similarity or Euclidean distance to compute the similarity between two semantic embeddings of $x_i$ and $x_j$ which depends on how the distance between data points and centroids is calculated during the partitioning. The more similar the semantic embeddings of two instruction inputs are, the more it means that the initial LLMs consider these two inputs to be of the same task category. So, when a submodel $M_i$ performs well on $\mathcal{N}_{xi}$, it's likely that it will provide accurate recommendations for $x_i$. Therefore, $M_i$ should be assigned a higher weight. We assign different weights to submodels $\{M_{0}, M_{1} ,..., M_{K} \}$based on their performance on $\mathcal{N}_{xi}$:
\begin{equation}\small 
w_{j} = \frac{exp(\alpha \cdot error(M_{j})) }{\sum_{l=0}^{K} exp(\alpha \cdot error(M_{l})) }  
\end{equation}

Where $w_{j}$ represents the attention weight that submodel $M_j$ needs to be assigned, and $\alpha$ is a hyper-parameter to control the importance of $error(M_{l}))$. $error(M_{l}))$ is defined as follow:
\begin{equation}\small 
error(M_{j}) = -\frac{1}{|\mathcal{N}_{x_i} |}\sum_{(x_l,y_l) \in \mathcal{N}_{x_i}} loss(M_{j}(x_l),y_l)  
\end{equation}
%Here $x_l$ and $y_l$ 分别代表了相似验证集中的 Instruction Input和 Instruction Output， loss是某种损失函数用于计算Mi对xl的生成结果和yl之间的差距，差距越小导致error(M_j)越大，故wj越大。

Here, $x_l$ and $y_l$ respectively represent the Instruction Input and Instruction Output in the similar validation set. The $loss$ is a certain loss function used to compute the gap between the generated result by $M_i$ for $x_l$ and the actual $y_l$. A smaller difference leads to a larger $error(M_{l})$, hence resulting in a higher $w_j$. With the obtained weights $\{w_{0},w_{1},...,w_{K}\}$ for an Instruction Input $x_i$ we can utilize equation~\ref{soup} or equation~\ref{cat} to create the model soup.

==> backup/4_exp.tex <==
\section{EXPERIMENTS}
In this section, we conduct a series of experiments to answer the following research questions:
\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1}: How does APA perform in terms of recommendation performance and unlearning efficiency compared to the state-of-the-art exact unlearning methods?
    \item \textbf{RQ2}: 
    % Can APA improve the inference efficiency compared to traditional prediction aggregation methods?
    How does APA perform in terms of inference efficiency?
    \item \textbf{RQ3}: How do the different components of APA affect its effectiveness?
\end{itemize}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[]
\caption{Comparison of different unlearning methods on recommendation performance, where `\textbf{APA(D)}'/`\textbf{APA(ND)}' represents APA implemented with decomposition/non-decomposition level aggregation, and $\bigtriangleup$ represents the gap between retraining and the unlearning method in terms of AUC. `Bef. Agg.' represents the average $AUC$ of the sub-model.}
\label{main}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Book}  & \textbf{Retraining} & \textbf{SISA} & \textbf{GraphEraser} & \textbf{RecEraser} & \textbf{APA(D)} & \textbf{APA(ND)} \\ \midrule
\textbf{Bef. Agg.}   & -           & 0.6561        & 0.6393                & 0.6525             & 0.6578
                 & 0.6578                \\\hdashline
\textbf{AUC}   & 0.6738           & 0.6731        & 0.6646                & 0.6719             & 0.6738                 & 0.6741                \\ 
\textbf{$\bigtriangleup$}  & -               & -0.0007        & -0.0092                & -0.0019             & 0                      & 0.0003                 \\
\midrule
\textbf{Movie} & \textbf{Retraining} & \textbf{SISA} & \textbf{GraphEraser} & \textbf{RecEraser} & \textbf{APA(D)} & \textbf{APA(ND)} \\ \midrule
\textbf{Bef. Agg.}   & -           & 0.7003        & 0.6732               & 0.6699             & 0.6874               & 0.6874                \\\hdashline
\textbf{AUC}   & 0.7428           & 0.7055        & 0.6885                & 0.6918             & 0.7171                 & 0.7172                \\
\textbf{$\bigtriangleup$}  & -                & -0.0373        & -0.0543                & -0.051              & -0.0257                 & -0.0256                \\ \bottomrule
\end{tabular}
\end{table*}

\subsection{Experimental Settings}
\subsubsection{Datasets}
We conduct experiments on two distinct real-world datasets, which are widely recognized and used within the realm of recommendation systems:
\begin{itemize}[leftmargin=*]
    \item \textbf{Movie}. We utilize the MovieLens100K~\cite{movielens} benchmark dataset, which comprises user ratings ranging from 1 to 5, following ~\cite{lightgcn,zhang2023reformulating}, we treat the ratings as ``like’’ (corresponding to the "Yes" in the TALLRec instruction out) if the ratings are higher than 3 and otherwise ``dislike’’. The dataset includes comprehensive textual attributes of the movies, such as ``title’’ and ``director''. We preprocess the original dataset by sampling the most recent 100,000 interactions and subsequently partitioning them into training, validation, and testing set, maintaining an 8:1:1 ratio. To construct recommendation instruction data, based on a user’s interacted item, ten items that the user has previously interacted with are retained as historical interactions.
    %To construct a recommendation instruction data. based on a user’s interacted item, ten items that the user has previously interacted with are retained as historical interactions. Then, we randomly select disjoint 1024 rec-tuning samples as training set, 1000 rec-tuning samples as validation set, and 500 rec-tuning samples as testing set. 
    \item \textbf{Book}. We utilize the BookCrossing dataset~\cite{bookcross}, which consists of user ratings ranging from 1 to 10. This dataset also provides textual descriptions of books, including attributes like ``book author'' and ``book title''. As this dataset lacks the timestamp information, so we construct a recommendation instruction sample by random sampling. Our approach involves randomly selecting one item that the user interacted with as the user's predicted target item. We then take the remaining 10 items that the user interacted with as the historical interactions for the target item. We divide the resulting dataset into training, validation, and testing set in an 8:1:1 ratio. Furthermore, we binarize the ratings based on a threshold of 5. Ratings exceeding 5 are considered as ``like'', while ratings below 5 are labeled as ``dislike''.
    %In the book domain, we leverage the BookCrossing dataset, which encompasses user ratings assigned to books on a scale ranging from 1 to 10. This dataset also includes textual descriptions of books, encompassing attributes such as "book author" and "book title." We randomly select one item that the user interacted with as the user's predicted target item, and take the remaining 10 items that the user interacted with as the historical interaction of the target item to construct a rec-tuning sample.  This sampling procedure is performed for each user within the original dataset, we divide the dataset into training, validation, and testing sets with the same ratio of 8:1:1. Additionally,we binarize the ratings according to a threshold of 5.
\end{itemize}
\subsubsection{Few-shot training Setting}
Following~\cite{tallrec}, we use few-shot training settings, where only a limited number of samples are randomly selected from the training set for model training. It has been demonstrated that even a small portion of the data can yield excellent recommendation performance. In this context, we follow~\cite{tallrec} and use ``1024-shot'' to represent the maximum learning size.
\subsubsection{Comparison of Methods}
Since we focus on exact machine unlearning, we compare with  traditional methods of exact machine unlearning as follows:

\begin{itemize}[leftmargin=*]
    \item \textbf{Retraining} represents the simplest and most direct approach, involving the removal of data to be forgotten, and then retraining the entire model. Nevertheless, it has a notable drawback in terms of substantial time overhead. % As such, it is included as the fundamental benchmark method.
    \item \textbf{SISA~\cite{sisa}} is a conventional machine unlearning method that involves random data partitioning of the training dataset into $K$ shards. Then $K$ sub-models are trained on each sub-dataset. Subsequently, at inference time, $K$ individual predictions from each sub-model are simply aggregated to provide a global prediction (\eg majority voting).
    \item \textbf{RecEraser~\cite{receraser}} is a machine unlearning method tailored specifically for recommendation systems. It incorporates three distinct data partitioning strategies,  splitting recommendation data into balanced shards. Additionally, RecEraser introduces an attention-based adaptive aggregation method to enhance performance. However, it is worth noting that the utilization of this attention-based adaptive aggregation method can lead to an increase in retraining time.
    \item \textbf{GraphEraser~\cite{graphunlearn}} is a state-of-the-art machine unlearning method designed for graph data. It utilizes node clustering techniques for graph partitioning such as bekm and blpa. Additionally, GraphEraser learns a static weighting scheme for aggregating the outputs of sub-models.

\end{itemize}

\subsubsection{Evaluation Metrics}
Given the intrinsic similarities between the current experimental setting and explicit recommendations, which pertain to the prediction of a user's level of interest in a particular target item, we employ the traditional explicit recommendation evaluation metric: the Area Under the Receiver Operating Characteristic (AUC)~\cite{tallrec} score as our primary evaluation criterion.

\subsubsection{Implementation Details}
%对于retrain的方法，我们使用‘1024-shot’的tallrec学习，tallrec的setting完全按照原文。我们将分组数k设置为4，对于SISA，我们将训练数据划分为4个大小为256的group，进行训练，对4个submodel的输出进行平均聚合。对于RecEraser，因为tallrec属于序列推荐，难以使用item-base和interaction-base的方法进行划分，我们只使用user-base的方法进行data partition。将每个rec-tuning samples当做一个特殊用户的user-item interaction，并构建interaction矩阵。使用MF（矩阵分解）的方法学习user embeddings，这里embedding大小为64, learning rate 为 5e-3. 在聚合层面难以使用attention的机制，故与SISA的方法类似，使用平均聚合。 在AdpterPS，对两个数据集我们分别使用了consine相似度和欧式距离去划分和寻找topk的验证集。对于consine相似度的方法，we set $\aplha=1500$ and $|\mathcal{N}_x| = 100$, 对于欧式距离的方法，we set $\aplha=200$ and $|\mathcal{N}_x| = 80$  
In our retraining method, we employ a ``1024-shot'' TALLRec model for learning, the remaining model parameters follow the original article~\cite{tallrec}. We set the number of shards $K$ to 4. As for the SISA method, we divided the training data into 4 groups, each with a size of 256, for training, and then averaged the outputs of the 4 sub-models. In the case of RecEraser, because TALLRec deals with a sequence recommendation task, using item-based and interaction-based methods for data partition is challenging. Instead, we exclusively utilized a user-based approach for the data partition. In this approach, each recommendation instruction data sample is treated as a distinct user's user-item interaction, and an interaction matrix is constructed. We employ the most representative CF model, matrix factorization (MF)~\cite{koren2009matrix} to learn user embeddings. The embedding size is set to 64, and the learning rate is configured at 5e-3. About GraphEraser, we utilize the Bekm method for data partitioning, similar to our semantic-aware approach, using hidden representations as representations for nodes. During the aggregation stage, both RecEraser and GraphEraser require the additional learning of aggregation parameters. Therefore, we adopt an average aggregation approach similar to SISA. For APA, in both datasets, we employ cosine similarity to partition the data and identify the top-n samples in the validation set. For the book dataset, we set $\alpha$ to 1500 and $|\mathcal{N}_{v}|$ to 100, and for the movie dataset, we set $\alpha$ to 300 and $|\mathcal{N}_{v}|$ to 20. And we conduct all experiments on the same machine(NVIDIA A40).
\subsection{Performace Comparison (\textbf{RQ1})}
\subsubsection{Accuracy Comparison}
%我们首先比较the recommendation accuracy of AdpterPS and baseline on TALLRec， which enables us to evaluate how our method maintains the recommendation performance. The comparison results are summarized in Table 2, where we have the following observations: 1) The retrain model shows better performance than SISA ，RecEraser。尤其是在movie数据集上，使用baseline的方法带来巨大的推荐效应的损失。since it uses the original dataset without the sample that need to be forgotten for training. However, as shown in the next section, its unlearning efficiency is low especially 甚至是在 few-shot的setting下 2）Our proposed AdpterPS achieves significantly better performance (p <0.01) than the state-of-the-art unlearning baselines on the two datasets. 尤其是在movie数据集上， AdpterPS 展示了 80%（todo）提升相对于于SISA，90%相对于RecEraser. 在book数据集上AdpterPS的方法不光能逼近甚至超过retrain model的performance。The substantial improvement could be attributed to two reasons: 1）AdpterPS partition data through  semantic embeddings which can enhance performance by making submodels heterogeneous。2）AdpterPS uses the proposed testing sample-adaptive approach 为每一个测试样本，we combine adapter weights based on its most semantically similar validation samples, using the validation performance of different adapters to assign aggregation weights。 3）可以发现两种层面的model soup均取得了相近的效果，在book数据集上 0.6687 和 0.6741 分别对应Lora parameters level model soup and Lora layers level model soup，在movie数据集上 0.7176 0.7207。可以解释为，这两种方法都是对LoRA的某一层进行聚合，所以达到的效果相近
We compare the accuracy of APA with that of the baselines on the two datasets in Table~\ref{main}, from which we have the following observations.
\begin{itemize}[leftmargin=*]
    \item  Both APA and prediction aggregation methods show improved $AUC$ compared to the $AUC$ of the best sub-model before aggregation. This indicates that the aggregated model itself has the ability to enhance overall model performance.
    \item The retraining model exhibits better performance than SISA, RecEraser, and GraphEraser. Particularly on the movie dataset, the baselines (\ie SISA, RecEraser, and GraphEraser) reveal a significant loss in recommendation performance. However, the unlearning efficiency of retraining is significantly low, even in the few shot settings (see evidence in Table~\ref{fig:time}), limiting its practical application. 
    \item Our proposed APA significantly outperforms ($p$ < 0.01) the state-of-the-art unlearning baselines on the two datasets. In particular,  on the movie dataset, the $AUC$ for APA(D) is 0.7172, while the corresponding result is 0.7055, 06885, and 0.6918  for the baselines (SISA, RecEraser, and GraphEraser) respectively. On the book dataset, APA not only approaches but even surpasses the performance of the retraining model. The substantial improvement can be attributed to several reasons: 1) APA partitions data through semantic embeddings, enhancing performance by making sub-models heterogeneous. 2) APA employs the proposed testing sample-adaptive approach. For each test sample, we combine adapter weights based on its most semantically similar validation samples, using the validation performance of different adapters to assign aggregation weights.
    \item We noted that both levels of the model aggregation produce similar results. On the book dataset, APA(D) achieves 0.6738 and APA(ND) achieves 0.6741. The same phenomenon also occurs in the movie dataset. This similarity can be attributed to the fact that both methods aggregate a specific layer of LoRA, resulting in similar outcomes.
\end{itemize}

%First, the retrain model exhibits better performance than SISA and RecEraser. Particularly on the movie dataset, using the baseline method incurs a significant loss in recommendation performance, as the retrain model uses the original dataset without the samples that need to be forgotten during training. However, as shown in the next section, its unlearning efficiency is low, even in the few-shot settings.

%Second, our proposed AdapterPS significantly outperforms (p < 0.01) the state-of-the-art unlearning baselines on the two datasets. Especially on the movie dataset, AdapterPS demonstrates an 80\% (to be confirmed) improvement compared to SISA and a 90\% improvement over RecEraser. On the book dataset, AdapterPS not only approaches but even surpasses the performance of the retrain model. The substantial improvement can be attributed to several reasons:1) AdapterPS partitions data through semantic embeddings, enhancing performance by making submodels heterogeneous.2) AdapterPS employs the proposed testing sample-adaptive approach. For each test sample, we combine adapter weights based on its most semantically similar validation samples, using the validation performance of different adapters to assign aggregation weights.


%Third, we noted that both levels of the model soup produced similar results. On the book dataset, the values of 0.6378 and 0.6741 correspond to the Lora parameters level model soup and Lora layers level model soup, respectively. On the movie dataset, the results are 0.7171 and 0.7172. This similarity can be attributed to the fact that both methods aggregate a specific layer of LoRA, resulting in similar outcomes.
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\subsubsection{Efficiency Comparison}
%\begin{table}[]
%\caption{Unlearning time}
%\begin{tabular}{@{}ccccc@{}}
%\toprule
%         & \multicolumn{2}{c}{book} & \multicolumn{2}{c}{movie} \\ \midrule
%retrain  & 61669s      &            & 40970s      &             \\
%AdpterPS & 16081s      & (3.83$\uparrow$)     & 10335s      & (3.96$\uparrow$)      \\ \bottomrule
%\end{tabular}
%\end{table}
%in this section，我们conduct 实验去explore the unlearning efficiency of our proposed method——AdpterPS. We randomly sample 100 rec-tuning samples 并从他们的Instruction Input中 随机remove一个user-item interaction。 使用新的rec-tuning samples训练新的retrain model，以及重新训练改变rec-tuning samples对应的submodel，训练submodel时我们采用并行训练。The shards number $K$ is set to 4, and all experiments are run on the same machine(to do A40).结果展示于table 3中，可以看出AdpterPS can significantly improve the unlearning efficiency。For example， 在movie数据集上，AdpterPS只用了10335s，并retrain的方法快了3.96倍。For retrain method, training on a large data is very timeconsuming. For our AdpterPS, only the corresponding submodel  need to be retrained to forget the required data。Moreover，与传统方法相比，我们的方法不需要花费多余时间去学习聚合的参数，验证集的效果在训练集中就已经被计算好。

We conduct experiments to explore the unlearning efficiency of our proposed method, APA. We randomly select 100 samples from the training set and remove one user-item interaction from their Instruction Input. We used these unlearning training set to train a new model, as well as to retraining corresponding sub-models affected by the changes.  The sub-model training was conducted in parallel. We set the number of shards $K$ to 4, and all experiments were conducted on the same machine (NVIDIA A40). The inference time of baselines and two APA variants is shown in Figure~\ref{fig:unlearntime}, indicating that APA significantly improves unlearning efficiency. For example, on the movie dataset, APA only took 10,335 seconds, making it 3.96 times faster than the retrain method. The retraining method is time-consuming as it is trained on the whole dataset. In contrast, APA only requires retraining the specific sub-model responsible for the unlearned data. Additionally, compared to traditional methods~\cite{receraser,graphunlearn}, APA does not necessitate extra time for learning aggregation parameters, as the validation set's performance is computed during the training process.

%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
%\begin{table}[]
%\caption{Inference time}
%\begin{tabular}{@{}ccc@{}}
%\toprule
%                       & \textbf{book} & \textbf{movie} \\ \midrule
%\textbf{Retrain}       & 47s           & 46s            \\
%\textbf{SISA}          & 187s          & 189s           \\
%\textbf{AdpterPS-cat}  & 58s           & 59s            \\
%\textbf{AdpterPS-soup} & 60s           & 59s            \\ \bottomrule
%\end{tabular}
%\end{table}
\begin{figure}
    \centering
    \subfigure[\textbf{Unlearning time}]{\label{fig:unlearntime}\includegraphics[width=0.22\textwidth]{unlearn_time.pdf}}
    \subfigure[ \textbf{Inference time}]{\label{fig:infre} \includegraphics[width=0.22\textwidth]{inferencetime.pdf}}
    \vspace{-15pt}    \caption{figure a: Unlearning time(seconde[s]) of Retrain and APA figure b: Inference time of Retrain, SISA, APA(D), and APA(ND)}
    \vspace{-15pt}
    \label{fig:time}
\end{figure}
\subsection{Inference Time Comparison (\textbf{RQ2})}
%在前一节的实验中我们已经studied our AdpterPS方法能为Unlearn节省大量时间。本节我们旨在探究ApterPS能否在推理阶段提升效率相较于output聚合方法。We randomly selected 500 Instruction Inputs from the testing set and tested the inference time 在这些样本上。这里为了符合实际情况——web application不会为一个服务api同时load 多个submodel，所以对output 聚合的方法需要依次进行多个sub model推理阶段，我们只统计推理阶段所需要时间。与4.2.2的效率实验相同，We set the number of shards $K$ to 4,所有实验均处于同意machine（A40）,实验结果如table4所示
In the previous section, we studied how our APA method can save a significant amount of time during the unlearning process. In this section, we examine whether APA can enhance efficiency during the inference stage compared to aggregation methods. We randomly select 500 Instruction Inputs from the testing set and measure the inference time for these samples. To align with real-world scenarios where web applications may not load multiple sub-models for a single service API simultaneously, we exclusively measure the time required during the inference stage for the predictions aggregation method. The experimental results are presented in Figure~\ref{fig:infre}. From the results, we have the following observations: 1) The results clearly show that while our method exhibits some gaps in time efficiency compared to using a single model directly for inference, the delay for a single user is approximately 0.02 seconds, which is entirely acceptable in real-world scenarios. 2) SISA's inference time is about 187s and 189s for the book and movie datasets, respectively. Our method significantly outperforms SISA in this regard. The additional time cost associated with using $K$ sub-models for inference is a primary reason for the observed inefficiency. The inference times for other predictions aggregation methods are similar to SISA so we omit them to save space. 3) It's worth noting that both APA(D) and APA(ND) achieve similar inference times. These results demonstrate that APA can achieve a high level of inference efficiency. %从结果可以看出，虽然我们的方法相对于直接使用一个model推理的时间效率存在差距，但是对一个single用户的delay大约时0.02s，在实际场景中完全可以接受。而SISA的推理时间需要about 187s，189s分别在book和movie数据集上，我们的方法要远远优于此。其他的output聚合的推理时间与SISA相近，故这里就不做展示。另外，可以注意到 the Lora parameters level model soup and the Lora layers level model soup可以达到相似的时间. 这些结果证明了AdpterPS可以达到较高的推理效率
\begin{figure}
    \centering
    \subfigure[\textbf{book}]{\label{fig:a}\includegraphics[width=0.22\textwidth]{datapartitionbook.pdf}}
    \subfigure[ \textbf{movie}]{\label{fig:b} \includegraphics[width=0.22\textwidth]{datapartitionmovie.pdf}}
    \vspace{-15pt}    \caption{Performance comparison of different data partition methods on book and movie datasets.}
    \vspace{-15pt}
    \label{fig:data-partition}
\end{figure}

\subsection{In-depth Studies(\textbf{RQ3})}
\subsubsection{Effect of the Proposed Data Partition Methods}
%为了去验证我们提出的data partition的有效性，我们compare with random分组, user-base分组, and  bekm~\cite{} 3种分组方法，并且都使用 testing sample-adaptive approach 进行modelsoup。图三展示了上述方法的performance。We can see that the proposed semantic data partition method can effectively improve the recommendation performance compared to random分组, user-base分组, and bekm，For exmaple on book dataset our method achieve 0.6738 of AUC score，while the corresponding result is 0.6503 for random分组 ， 0.6627 for user-base分组 and 0.6411 for bekm, respectively.
To validate the effectiveness of our proposed data partition method, we compare it with three other grouping methods: random partition, user-based partition, and BEKM partition~\cite{graphunlearn}. We apply the sample-adaptive approach to all methods. The experimental findings are illustrated in Figure~\ref{fig:infre}. Based on the results, we've made the following observations: 1) the proposed semantic data partition method significantly improves recommendation performance compared to random partition, user-based partition, and BEKM. For example, on the book dataset, our method achieve an AUC score of 0.6738, while the corresponding results were 0.6503, 0.6627, and 0.6411 for random partition, user-based partition, and BEKM, respectively. 2) The user-based partition method performs poorly on both datasets, suggesting that LLM might not comprehend traditional recommendation information and has a negative impact on the entire grouping. 3) It is worth noting that the random partition method achieves results close to our method on the movie dataset. This is because the random partition method happening to create sub-models that align well with our weighted approach. 
\begin{figure}
    \centering
    \subfigure[\textbf{book}]{\label{fig:a}\includegraphics[width=0.22\textwidth]{aggbook.pdf}}
    \subfigure[ \textbf{movie}]{\label{fig:b} \includegraphics[width=0.22\textwidth]{aggmovie.pdf}}
    \vspace{-15pt}    \caption{Performance comparison of different data partition methods on book and movie datasets.}
    \vspace{-15pt}
    \label{fig:agg}
\end{figure}

\subsubsection{Effect of the Proposed Sample-adaptive Method}
%Next，we evaluate the model utility of different 权重方法以此证明我们proposed testing sample-adaptive method的有效性。我们比较的方法有平均model soup，以及major-base的方法 which 对每一个test sample我们只选择权重最大的一个sub model进行推理预测·实验结果见表4，We can observe that , the mean model soup is far less than the one considering testing sample-adaptive method, especially for movie dataset。另一个值得注意的是只使用权重的submodel虽然可以保持较高的推荐效果，但是与我们的方法还是存在差距。原因是我们的方法考虑了其他submodel的信息，鲁棒和泛化性更好。This verifies,Using our proposed method helps better capture the global structural information by assigning different weights to shard models.
We proceed to assess the model utility of different weight methods to demonstrate the effectiveness of our proposed testing sample-adaptive method. We compare the mean model aggregation~\cite{modelsoup} and the major-based method~\cite{sisa}. In the major-based approach, for each testing sample, we only select the sub-model with the highest weight for inference prediction. Additionally, we evaluate the test-based method, which calculates weights for each testing sample without utilizing validation set information. Instead, it calculates weights based on the similarity between the sample and the centroids of different shards. ALL these models are combined with Semantic-aware Data Partition. The experimental results are presented in Table~\ref{fig:agg}. Here are some observations we found: 1) The mean model aggregation underperforms APA on both datasets. This is because mean model aggregation fails to leverage the heterogeneity of sub-models effectively. Treating each sub-model equally results in a decrease in performance. 2) The test-based method also exhibits lower recommendation performance compared to APA, confirming the effectiveness of utilizing validation set information. 3) Another noteworthy point is that using only the highest-weighted sub-model can maintain relatively high recommendation performance, but there is still a gap compared to our method. The reason for this difference is that our method considers information from other sub-models, making it more robust and generalizable. This demonstrates that using our proposed method helps capture global structural information more effectively by assigning different weights to shard models.

\subsubsection{Impact of the Shard Size}
%We conducted the experiments only on the book dataset in order to study the impact of the shard number.我们将分组设置为{2，4，8}并进行了unlearn效率和推荐效果的evaluate。实验结果如图4所示，可以看出在unlearn时间随着k的增大逐步奸杀。This makes sense as a larger number of shards means a smaller shard size, which will improve the unlearning efficiency。但是伴随着shards数量的增多，推荐效应逐步下降，for example在K=2时，AUC达到了0.6786 和 0.6783 分别对应 AdpterPS-soup 和 Adpter-cat，甚至比retrain model的效果好，但是当K=8时，效果急剧下降。这可能是因为shards增多，我们的 testing sample-adaptive method 难以捕捉到每个模块的特点，导致聚合效果变差。 In practice, The number of shards should be carefully selected to balance the unlearning efficiency and recommendation performance.
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{shardsbook.pdf}
   \vspace{-10pt}
  \caption{Impact of the shard number on the unlearning efficiency and performance on book datasets. The bar chart shows the recommendation performance and the line chart shows the unlearning time cost.}
  \label{fig:shard}\vspace{-15pt}
\end{figure}
We investigate the influence of the shard size on the book dataset. We configure the shrad size as $\{512, 256, 128\}$ and evaluate unlearning efficiency and recommendation performance. The experimental results are displayed in Figure~\ref{fig:shard}. The increase in shard size corresponds to a gradual rise in unlearning time. This is anticipated as larger shard sizes lead to longer retraining periods for each sub-model, directly impacting the efficiency of unlearning. However, with a decrease in the shard size, the recommendation performance gradually declines. For instance, when shard size is 512, the $AUC$ reached 0.6786 and 0.6783 for APA(D) and APA(ND), respectively, even surpassing the retrain model's performance. But when shard size is 128, there is a significant drop in performance. This could be attributed to the following factors: 1) Reducing the shard size means an increase in the number of sub-models $K$. This adjustment might pose a challenge for our testing sample-adaptive method in accurately capturing the unique characteristics of each shard. As a result, the aggregation results could suffer. 2) Smaller shard sizes can naturally lead to reduced performance in individual sub-models, consequently affecting the overall effectiveness of the aggregated model. In practice, the shards should be thoughtfully chosen to strike a balance between unlearning efficiency and recommendation performance.

==> backup/6_related.tex <==
\section{Related work}
\noindent \textbf{Machine unlearning.} %当一个模型被训练好之后，它会记住information of training data。在许多实际场景中，需要model有能过遗忘这些information的能力，eg。。The task is called machine unlearning, and there appear two types of methods: approximate unlearning and exact unlearning。 前者的方法尽量让模型与retrain model表现相似，这类工作通过避免重新训练模型的方式，以获得more efficient and less costly unlearning。 多数的方法通过基于梯度的方法进行参数去消除需要unlearn的数据给模型带来的影响
When a model is trained, it retains the information from the training data. However, in many real-world scenarios, there is a need for a model to have the ability to forget this information, e.g.privacy~\cite{cao2015towards} and security~\cite{marchant2022hard}. This task is known as machine unlearning, and it involves two main types of methods~\cite{unlearninSurvey,anothersurvey}: approximate unlearning and exact unlearning. Approximate unlearning methods aim to make the model's performance similar to that of a retrained model. These approaches seek to mitigate the impact of data that needs to be forgotten on the model without retraining, leading to more efficient and cost-effective unlearning. Most of these methods rely on gradient-based techniques~\cite{ifru,guo2019certified,neel2021descent,izzo2021approximate} to remove the influence of the data that needs to be unlearned on the model's parameters.  

Exact unlearning methods guarantee the removal of the data that needs to be forgotten from the model. Early works in this area have focused on simple models and specific cases. For example, work ~\cite{cao2015towards} delves into exact unlearning using statistical queries for Naive Bayes classifiers, while work ~\cite{ginart2019making} focuses on deletion algorithms for k-means clustering. Recent work on exact unlearning has predominantly centered around the data-partition framework proposed by SISA~\cite{sisa}. This framework involves three key steps: 1) dividing the training data into disjoint shards, 2) training distinct submodels for each shard, and 3) aggregating K individual predictions from each submodel to provide a global prediction. Similar works include~\cite{yan2022arcane, qian2022patient, receraser, graphunlearn}. They employ various partitioning and aggregation methods to achieve improved predictions based on their specific task scenarios. However, this paradigm is challenging to apply to LLM4Rec unlearning, primarily because of the computationally expensive nature of LLM inference~\cite{costhigh}. Generating predictions from K sub-models would significantly increase the inference cost of LLMs, which is unacceptable in practical industrial settings.

\noindent \textbf{LLMunlearning.}%目前LLMUnlearn的工作都可以被分为approximate unlearn。For exmaple，~\cite{HarryUnlearning}通过比较强化特定知识模型和通用模型，识别与unlearn目标相关的token，替换Unlearn目标特殊文本为通用文本，生成finetune data，并微调模型。 ~\cite{yao2023large}使用了一种结合LLMS特点的Gradinet Ascent进行参数更新。 ~\cite{InContextUnlearn}则是使用类似In-context learn的机制去eliminate the influence of an unlearn training point on the model output.这些工作均不能应用于LLM4Rec Unlearning的场景，因为他们不能保证把某个用户的隐私数据完全删除，可能还会存在隐私泄露的风险。
Currently, most Large Language Model (LLM) unlearning methods fall under the category of approximate unlearning. For instance, in the paper by the authors~\cite{HarryUnlearning}, they identify tokens related to the unlearn target by comparing specialized knowledge models with general models. They replace the specific text related to the unlearn target with generic text, generate fine-tuning data, and fine-tune the model. In another work~\cite{yao2023large}, a Gradient Ascent method that combines the characteristics of LLMs is used for parameter updates. In~\cite{InContextUnlearn}, a mechanism similar to in-context learning is employed to eliminate the influence of an unlearn training point on the model's output. However, these methods may not be suitable for LLM4Rec unlearning scenarios because they cannot guarantee the complete removal of a user's private data, potentially posing privacy risks.

\noindent \textbf{Model Soup.}%model soup最开始可以被称为averaging model weights，早期的一些工作~\cite{}weight-average models which share an initialization but are optimized independently.~\cite{modelsoup}将这一方法运用在pretrain and finetuning的模型上，并提出model soup这一概念。这种model soup的方法就是我们Lora parameters level model soup的方法相似。后续~\cite{}将 model soup 用于  averaging weights of newly-added parameters for parameter-efficient fine-tuning。但是~\cite{}与本文不同是，他们对peft parameters采用平均聚合，但是我们的方法对不同的peft采用不同参数，以达到好的推荐效果。 同样MoE(Mixture-of-Experts) 也可以用来model soup，这种方法与我们的Lora layers level model soup相似。只不过每个PEFT的weight用GATE机制计算，需要额外训练一部分参数。目前已有工作将MoE应用于peft范式的下的LLM。但是这种方法，是不适合unlearn场景的，因为unlearn 子模型后，还需要花费多余时间去训练MoE的相关参数，而我们的方法不需要。
The concept of model soup, initially termed "averaging model weights," has its roots in previous works such as~\cite{frankle2020linear,andreassen2021evolution}, where models share an initialization but are optimized independently. Later, the idea of model soup was introduced by ~\cite{modelsoup} applying this method to pretraining and fine-tuning models. This model soup method aligns with our Lora parameters level model soup approach. Recently, ~\cite{adamix} employed model soup for averaging the weights of newly added parameters during parameter-efficient fine-tuning. However, it differs from our approach in that they use average aggregation for PEFT parameters, while our method adjusts parameters differently for various PEFTs to achieve better recommendation performance.

Additionally, Mixture-of-Experts (MoE)~\cite{MoE} can also be employed for the model soup, resembling our Lora layers level model soup approach. In this method, each PEFT's weight is calculated using a GATE mechanism, requiring additional parameter training. There are some works~\cite{wang2023mt4crossoie,diao2023mixture} that have applied MoE to LLMs under the PEFT paradigm. However, this approach may not be suitable for unlearning scenarios because, after unlearning submodels, additional time is needed to train the related MoE parameters, while our method does not require this.

